BAGS: Blur Agnostic Gaussian Splatting through Multi-Scale Kernel Modeling

Recent efforts in using 3D Gaussians for scene reconstruction and novel view synthesis can achieve impressive results on curated benchmarks; however, images captured in real life are often blurry. In this work, we analyze the robustness of Gaussian-Splatting-based methods against various image blur, such as motion blur, defocus blur, downscaling blur, \etc. Under these degradations, Gaussian-Splatting-based methods tend to overfit and produce worse results than Neural-Radiance-Field-based methods. To address this issue, we propose Blur Agnostic Gaussian Splatting (BAGS). BAGS introduces additional 2D modeling capacities such that a 3D-consistent and high quality scene can be reconstructed despite image-wise blur. Specifically, we model blur by estimating per-pixel convolution kernels from a Blur Proposal Network (BPN). BPN is designed to consider spatial, color, and depth variations of the scene to maximize modeling capacity. Additionally, BPN also proposes a quality-assessing mask, which indicates regions where blur occur. Finally, we introduce a coarse-to-fine kernel optimization scheme; this optimization scheme is fast and avoids sub-optimal solutions due to a sparse point cloud initialization, which often occurs when we apply Structure-from-Motion on blurry images. We demonstrate that BAGS achieves photorealistic renderings under various challenging blur conditions and imaging geometry, while significantly improving upon existing approaches.

==> camera_motion_results.tex <==
\begin{table*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{

    \begin{tabular}{l |ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc}

     Camera  & \multicolumn{3}{c|}{NeRF}  & \multicolumn{3}{c|}{Mip-Splatting} &  \multicolumn{3}{c|}{Deblur-NeRF}  & \multicolumn{3}{c|}{DP-NeRF} & \multicolumn{3}{c|}{BAD-NeRF} & \multicolumn{3}{c|}{ExbluRF} & \multicolumn{3}{c|}{PDRF} & \multicolumn{3}{c}{Robust-GS (ours)}  \\

     Motion& PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS\\

     \midrule[1pt]

    
    Ball & 24.08 & 0.624 & 0.399 & 23.22 & 0.619 & 0.340 & 27.36 & 0.766 & 0.223 & 27.20 & 0.765 & 0.209 & 20.61 &.452 &.516 & 28.35 & 0.791 & 0.205 & 27.88 & 0.783 & 0.209 & 27.68 & 0.799 & 0.150\\
    Basket & 23.72 & 0.709 & 0.322 & 23.24 & 0.688 & 0.288 & 27.67 & 0.845 & 0.148 & 27.74 & 0.846 & 0.129 & 16.24 &.304 &.533 & 28.86 & 0.875 & 0.126 & 28.63 & 0.869 & 0.119 & 29.54 & 0.900 & 0.068 \\
    Buick & 21.59 & 0.633 & 0.350 & 21.46 & 0.658 & 0.266 & 24.77 & 0.770 & 0.175 & 25.70 & 0.792 & 0.141 & 13.40 &.159 &.623 & 25.95 & 0.809 & 0.154 & 25.69 & 0.790 & 0.165 & 26.18 & 0.844 & 0.088 \\
    Coffee & 26.48 & 0.806 & 0.290 & 24.73 & 0.749 & 0.288 & 30.93 & 0.898 & 0.124 & 31.19 & 0.905 & 0.100 & 21.38 &.566 &.546 & 32.44 & 0.915 & 0.101 & 32.41 & 0.913 & 0.112 & 31.59 & 0.908 & 0.096 \\
    Decoration & 22.39 & 0.661 & 0.363 & 20.55 & 0.641 & 0.299 & 24.19 & 0.771 & 0.186 & 24.31 & 0.781 & 0.164 & 14.85 &.177 &.776 & 23.51 & 0.740 & 0.275 & 23.29 & 0.734 & 0.228 & 26.09 & 0.858 & 0.083 \\
    Girl & 20.07 & 0.708 & 0.320 & 19.87 & 0.714 & 0.278 & 22.27 & 0.798 & 0.169 & 23.33 & 0.814 & 0.150 & 14.97 &.329 &.647 & 21.80 & 0.770 & 0.205 & 23.94 & 0.830 & 0.171 & 25.45 & 0.869 & 0.079 \\
    Heron & 20.50 & 0.522 & 0.413 & 19.43 & 0.505 & 0.332 & 22.63 & 0.687 & 0.210 & 22.88 & 0.693 & 0.191 & 15.86 &.189 &.544 & 22.52 & 0.676 & 0.281 & 22.84 & 0.692 & 0.231 & 22.04 & 0.715 & 0.126 \\
    Parterre & 23.14 & 0.620 & 0.405 & 22.28 & 0.590 & 0.321 & 25.82 & 0.760 & 0.216 & 25.86 & 0.767 & 0.190 & 17.20 &.234 &.656 & 24.97 & 0.768 & 0.227 & 25.64 & 0.758 & 0.235 & 25.92 & 0.819 & 0.092 \\
    Puppet & 22.09 & 0.609 & 0.339 & 22.05 & 0.631 & 0.267 & 25.24 & 0.751 & 0.158 & 25.25 & 0.754 & 0.151 & 14.99 &.214 &.669 & 25.12 & 0.758 & 0.181 & 24.99 & 0.761 & 0.147 & 25.81 & 0.804 & 0.094 \\
    Stair & 22.87 & 0.456 & 0.487 & 21.91 & 0.474 & 0.387 & 25.39 & 0.630 & 0.210 & 25.59 & 0.635 & 0.177 & 16.89 &.137 &.649 & 25.78 & 0.647 & 0.229 & 25.73 & 0.639 & 0.211 & 26.69 & 0.721 & 0.080 \\

    \midrule[1pt]
    
    Average & 22.69 & 0.635 & 0.369 & 21.87 & 0.627 & 0.306 & 25.63 & 0.767 & 0.182 & 25.91 & 0.775 & 0.160 & 16.64 &.276 &.616 & 25.93 & 0.775 & 0.198 & 26.10 & 0.777 & 0.183 & 26.70 & 0.824 & 0.096 \\
    \end{tabular}
}    
    \label{tab:results_motion}
    \caption{Quantitative Comparisons on the camera motion blur.}
    
\end{table*}


==> defocus_results.tex <==
\begin{table*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{

    \begin{tabular}{l |ccc|ccc|ccc|ccc|ccc|ccc}

     \multicolumn{1}{c|}{\multirow{2}[0]{*}{Defocus}}  & \multicolumn{3}{c|}{NeRF}  & \multicolumn{3}{c|}{Mip-Splatting} &  \multicolumn{3}{c|}{Deblur-NeRF}  & \multicolumn{3}{c|}{DP-NeRF} & \multicolumn{3}{c|}{PDRF} & \multicolumn{3}{c}{Robust-GS (ours)}  \\

     & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\

     \midrule[1pt]
     
    Cake & 24.42 & 0.721 & 0.225 & 22.17 & 0.645 & 0.290 & 26.27 & 0.780 & 0.128 & 26.16 & 0.778 & 0.127 & 27.07 & 0.799 & 0.120 & 27.21 & 0.818 & 0.108 \\
    Caps & 22.73 & 0.631 & 0.280 & 21.00 & 0.503 & 0.442 & 23.87 & 0.713 & 0.161 & 23.95 & 0.712 & 0.143 & 24.10 & 0.716 & 0.147 & 24.16 & 0.725 & 0.159 \\
    Cisco & 20.72 & 0.722 & 0.126 & 20.08 & 0.709 & 0.163 & 20.83 & 0.727 & 0.087 & 20.73 & 0.726 & 0.084 & 20.55 & 0.725 & 0.091 & 20.79 & 0.743 & 0.070 \\
    Coral & 19.81 & 0.566 & 0.269 & 19.60 & 0.555 & 0.323 & 19.85 & 0.600 & 0.121 & 22.80 & 0.741 & 0.096 & 19.53 & 0.591 & 0.112 & 20.53 & 0.628 & 0.117 \\
    Cupcake & 21.88 & 0.681 & 0.216 & 21.55 & 0.681 & 0.213 & 22.26 & 0.722 & 0.116 & 20.11 & 0.611 & 0.118 & 23.09 & 0.754 & 0.094 & 22.93 & 0.762 & 0.080 \\
    Cups & 25.02 & 0.758 & 0.232 & 20.93 & 0.646 & 0.314 & 26.21 & 0.799 & 0.127 & 26.75 & 0.814 & 0.104 & 26.28 & 0.812 & 0.127 & 26.27 & 0.823 & 0.104 \\
    Daisy & 22.74 & 0.620 & 0.262 & 21.59 & 0.614 & 0.273 & 23.52 & 0.687 & 0.121 & 23.79 & 0.697 & 0.108 & 24.39 & 0.741 & 0.091 & 23.74 & 0.746 & 0.062 \\
    Sausage & 17.79 & 0.483 & 0.279 & 17.78 & 0.473 & 0.284 & 18.01 & 0.500 & 0.180 & 18.35 & 0.544 & 0.147 & 18.86 & 0.564 & 0.143 & 18.76 & 0.574 & 0.110 \\
    Seal & 22.79 & 0.627 & 0.268 & 22.13 & 0.592 & 0.310 & 26.04 & 0.777 & 0.105 & 25.95 & 0.778 & 0.103 & 26.47 & 0.806 & 0.084 & 26.52 & 0.812 & 0.090 \\
    Tools & 26.08 & 0.852 & 0.155 & 23.98 & 0.812 & 0.196 & 27.81 & 0.895 & 0.061 & 28.07 & 0.898 & 0.054 & 28.14 & 0.901 & 0.059 & 28.60 & 0.913 & 0.046 \\
    
    \midrule[1pt]
    Average & 22.40 & 0.666 & 0.231 & 21.08 & 0.623 & 0.281 & 23.47 & 0.720 & 0.121 & 23.67 & 0.730 & 0.108 & 23.85 & 0.741 & 0.107 & 23.95 & 0.754 & 0.095 \\

    \end{tabular}
}
    \label{tab:results_defocus}
    \caption{Quantitative Comparisons on the defocus blur.}
    
\end{table*}





==> defocus_results_vis.tex <==
% %& $\textrm{XraySyn}_{ref}$ 
% \captionsetup[subfigure]{labelformat=empty}
% \begin{figure*}[htb!]
%     % \setlength{\abovecaptionskip}{3pt}
%     \setlength{\tabcolsep}{0.5pt}
%     \centering
%     \small
%     \begin{tabular}[b]{cccccccc}
%         % \hline
%          Novel View & NeRF & \tiny{Mip-Sp} & Db & DP & PDRF & Ours & G.T.\\
        
%         %%%%%%%%% defocus cupcake
%         \begin{subfigure}[b]{0.21\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/cupcake/000_defocuscupcake_gt.png}
%             \caption{PSNR/SSIM}
%         \end{subfigure} 
%         &  
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/cupcake/000_defocuscupcake_nerf_cut.png}
%             \caption{}
%         \end{subfigure}
%         &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/cupcake/000_defocuscupcake_mipsp_cut.png}
%             \caption{20.55/.641}
%         \end{subfigure} 
%         &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/cupcake/000_defocuscupcake_deblur_nerf_cut.png}
%             \caption{24.19/.771}
%         \end{subfigure} 
%         &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/empty.png}
%             \caption{}
%         \end{subfigure}
%         &   
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/cupcake/000_defocuscupcake_pdrf_cut.png}
%             \caption{23.29/.734}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/cupcake/000_defocuscupcake_ours_cut.png}
%             \caption{26.09/.858}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/cupcake/000_defocuscupcake_gt_cut.png}
%             \caption{}
%         \end{subfigure}\\ 


%         %%%%%%%%% defocus tools
%         \begin{subfigure}[b]{0.21\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/tools/005_defocustools_gt.png}
%             \caption{PSNR/SSIM}
%         \end{subfigure} 
%         &  
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/empty.png}
%             \caption{}
%         \end{subfigure}
%         &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/tools/005_defocustools_mipsp_cut.png}
%             \caption{20.55/.641}
%         \end{subfigure} 
%         &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/tools/005_defocustools_deblur_nerf_cut.png}
%             \caption{24.19/.771}
%         \end{subfigure} 
%         &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/empty.png}
%             \caption{}
%         \end{subfigure}
%         &   
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/tools/005_defocustools_pdrf_cut.png}
%             \caption{23.29/.734}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/tools/005_defocustools_ours_cut.png}
%             \caption{26.09/.858}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.108\linewidth}
%             \includegraphics[width=\textwidth]{figs/results_vis/Defocus/tools/005_defocustools_gt_cut.png}
%             \caption{}
%         \end{subfigure}\\ 


%     \end{tabular}
%     \caption{Visual comparisons of different scene reconstruction methods. }
%     \label{tab:visualization}

% \end{figure*}


==> intro_figure.tex <==
\begin{figure}[!htb]
\captionsetup{font=scriptsize}
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{0.1}
    \centering
    \begin{tabular}[b]{ccc}
         \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/deblur_crop.png}
            % \caption{DAMS}
            \label{img:deblur}
        \end{subfigure} &
         \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/gt_crop.png}
            % \caption{Ground Truth}
            \label{img:gt}
        \end{subfigure} &
        
        % \multirow{2}[0]{*}{
        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/blurball_019.jpg}
            % \caption{Input Image}
            \label{img:input}
        \end{subfigure}
        % } % 让我等下查查这个怎么弄

        
        \\

        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/deblur_cut.png}
            \caption{Robust-GS}
            \label{img:deblurcut}
        \end{subfigure} &
        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/gt_cut.png}
            \caption{Ground Truth}
            \label{img:gtcut}
        \end{subfigure} &
        
        \\
        
        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/nerfacto_crop.png}
            % \caption{Nerfacto}
            \label{img:nerfacto}
        \end{subfigure} &
        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/mipsp_crop.png}
            % \caption{Mip-Splatting}
            \label{img:mipsp}
        \end{subfigure} &

        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/horbar.png}
            \label{img:horbar}
        \end{subfigure} 
        
        \\
        
        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/nerfacto_cut.png}
            \caption{NeRFacto}
            \label{img:nerfactocut}
        \end{subfigure} &
        \begin{subfigure}[b]{.19\linewidth}
            \includegraphics[width=\textwidth]{figs/intro/mipsp_cut.png}
            \caption{Mip-Splatting}
            \label{img:mipspcut}
        \end{subfigure} &      
        \\
    \end{tabular}
    \caption{}
    \label{fig:intro}
    % \vspace{-0.5em}
\end{figure}






==> mask_kernel_vis_bu.tex <==
\begin{figure}[!htb]
    % \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.3\linewidth}
            \includegraphics[width=\textwidth]{figs/mask_kernel_vis/stair_blur_image.png}
            \caption{}
            \label{img:mrori}
        \end{subfigure} &
        \begin{subfigure}[b]{.4\linewidth}
            \includegraphics[width=\textwidth]{figs/mask_kernel_vis/stair_kernel_mask.pdf}
            \caption{}
            \label{}
        \end{subfigure} \\
        
        \begin{subfigure}[b]{.3\linewidth}
            \includegraphics[width=\textwidth]{figs/mask_kernel_vis/cupcake_blur_image.png}
            \caption{}
            \label{img:DSK}
        \end{subfigure} &
        \begin{subfigure}[b]{.4\linewidth}
            \includegraphics[width=\textwidth]{figs/mask_kernel_vis/cupcake_kernel_mask.pdf}
            \caption{}
            \label{img:PRE}
        \end{subfigure} \\

        \begin{subfigure}[b]{.3\linewidth}
            \includegraphics[width=\textwidth]{figs/mask_kernel_vis/bonsai_blur_image.png}
            \caption{}
            \label{img:DSK}
        \end{subfigure} &
        \begin{subfigure}[b]{.4\linewidth}
            \includegraphics[width=\textwidth]{figs/mask_kernel_vis/bonsai_kernel_mask.pdf}
            \caption{}
            \label{img:PRE}
        \end{subfigure} \\
        
    \end{tabular}
    % \caption{}
    \label{fig:pre}

\end{figure}

==> mip.tex <==

\begin{table}
\centering

\begin{tabular}{l l | l | l l | l | l l c l l | l | l l c l}
 &  & NeRFacto &  &  & Mip-NeRF 360 &  &  & Mip-Sp &  &  & Mip-Sp-Deblur &  &  & Ours &  \\
 & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\


\end{tabular}

\end{table}


==> mip360_compression_results.tex <==
\begin{table*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{

    \begin{tabular}{l |ccc|ccc|ccc|ccc|ccc}

     \multicolumn{1}{c|}{\multirow{2}[0]{*}{Compression}}  & \multicolumn{3}{c|}{NeRFacto}  & \multicolumn{3}{c|}{Mip-NeRF 360} &  \multicolumn{3}{c|}{Mip-Splatting}  & \multicolumn{3}{c|}{Mip-Splatting (SR)} & \multicolumn{3}{c}{Robust-GS (ours)}  \\

     & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\

     \midrule[1pt]

     Bicycle &  &  &  &  &  &  & 24.43 & 0.623 & 0.391 & 24.34 & 0.604 & 0.413 & 24.58 & 0.638 & 0.283 \\
    Bonsai &  &  &  &  &  &  & 27.72 & 0.816 & 0.291 & 28.05 & 0.823 & 0.285 & 27.06 & 0.818 & 0.173 \\
    Counter &  &  &  &  &  &  & 26.66 & 0.789 & 0.296 & 26.87 & 0.799 & 0.287 & 26.52 & 0.793 & 0.191 \\
    Flowers &  &  &  &  &  &  & 21.84 & 0.553 & 0.428 & 21.82 & 0.554 & 0.422 & 21.88 & 0.581 & 0.356 \\
    Garden &  &  &  &  &  &  & 25.04 & 0.632 & 0.398 & 25.02 & 0.631 & 0.403 & 25.42 & 0.672 & 0.323 \\
    Kitchen &  &  &  &  &  &  & 26.21 & 0.712 & 0.330 & 26.43 & 0.731 & 0.318 & 26.59 & 0.749 & 0.216 \\
    Room &  &  &  &  &  &  & 29.10 & 0.855 & 0.297 & 29.44 & 0.858 & 0.290 & 28.95 & 0.861 & 0.169 \\
    Stump &  &  &  &  &  &  & 25.40 & 0.654 & 0.389 & 25.55 & 0.658 & 0.385 & 25.27 & 0.662 & 0.237 \\
    Treehill &  &  &  &  &  &  & 22.67 & 0.533 & 0.482 & 22.58 & 0.531 & 0.483 & 22.49 & 0.539 & 0.375 \\

    \midrule[1pt]
    Average &  &  &  &  &  &  & 25.45 & 0.685 & 0.367 & 25.57 & 0.687 & 0.365 & 25.42 & 0.701 & 0.258 \\



\end{tabular}
}
\end{table*}






==> mixedres_illustration.tex <==
\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.18\linewidth}
            \includegraphics[width=\textwidth]{figs/mixedres_illustration/original_cut_noredbound.png}
            \caption{}
            \label{img:mrori}
        \end{subfigure} &
        \begin{subfigure}[b]{.18\linewidth}
            \includegraphics[width=\textwidth]{figs/mixedres_illustration/2x_cut_noredbound.png}
            \caption{}
            \label{}
        \end{subfigure} \\
        
        \begin{subfigure}[b]{.18\linewidth}
            \includegraphics[width=\textwidth]{figs/mixedres_illustration/3x_cut_noredbound.png}
            \caption{}
            \label{img:DSK}
        \end{subfigure} &
        \begin{subfigure}[b]{.18\linewidth}
            \includegraphics[width=\textwidth]{figs/mixedres_illustration/4x_cut_noredbound.png}
            \caption{}
            \label{img:PRE}
        \end{subfigure} \\
        
    \end{tabular}
    \caption{}
    \label{fig:pre}

\end{figure}
